Outsourcing an Information Operation: A Complete Dataset of Tenet Media's Podcasts on Rumble

Tenet Media, a U.S.-based, right-wing media company, hired six established podcasters to create content related to U.S. politics and culture during the 2024 U.S. presidential election cycle. After publishing content on YouTube and Rumble for nearly a year, Tenet Media was declared by the U.S. government to be funded entirely by Russia -- making it effectively an outsourced state-sponsored information operation (SSIO). We present a complete dataset of the 560 podcast videos published by the Tenet Media channel on the video-sharing platform Rumble between November 2023 and September 2024. Our dataset includes video metadata and user comments, as well as high-quality video transcriptions, representing over 300 hours of video content. This dataset provides researchers with material to study a Russian SSIO, and notably on Rumble, which is an understudied platform in SSIO scholarship.

==> edits.tex <==
% \begin{table}[t]
% \begin{tabular}{rl}
% \multicolumn{1}{l}{\textbf{Topic}} & \textbf{Topic Words}                                         \\ \hline
% \multicolumn{1}{r|}{0}             & case, trump, court, question, law,              \\
% \multicolumn{1}{r|}{}              & tim, biden, guy, government, says               \\ \cline{2-2} 
% \multicolumn{1}{r|}{1}             & gay, guys, white, media, different,             \\
% \multicolumn{1}{r|}{}              & gender, kids, culture, opinion, month            \\ \cline{2-2} 
% \multicolumn{1}{r|}{2}             & dave, love, years, guy, kids,                   \\
% \multicolumn{1}{r|}{}              & today, isabel, whats, laughing, guys             \\ \cline{2-2} 
% \multicolumn{1}{r|}{3}             & black, israel, crowd, chicago, vote,            \\
% \multicolumn{1}{r|}{}              & money, white, riot, booing, reparations          \\ \cline{2-2} 
% \multicolumn{1}{r|}{4}             & canada, government, canadian, canadians,          \\
% \multicolumn{1}{r|}{}              & housing, years, trudeau, covid, money, country \\ \cline{2-2} 
% \multicolumn{1}{r|}{5}             & women, men, kids, school, white,                \\
% \multicolumn{1}{r|}{}              & years, guys, woman, world, work                  \\ \cline{2-2} 
% \multicolumn{1}{r|}{6}             & case, court, law, gun, crime,                   \\
% \multicolumn{1}{r|}{}              & police, amendment, federal, guns, judge         \\ \cline{2-2} 
% \multicolumn{1}{r|}{7}             & trump, biden, joe, president, donald,           \\
% \multicolumn{1}{r|}{}              & country, kamala, party, man, harris             \\ \cline{2-2} 
% \multicolumn{1}{r|}{8}             & congress, trump, house, president, committee,   \\
% \multicolumn{1}{r|}{}              & members, staff, office, donald, military        
% \end{tabular}
% \caption{Topic modeling analysis of video transcripts.}
% \label{Table 2}
% \end{table}


% \begin{table*}[]
% \begin{tabular}{lll|lll|lll|ll}
% \multicolumn{3}{l|}{\textbf{Video Title Named Entities}} & \multicolumn{3}{l|}{\textbf{Video Description Named Entities}} & \multicolumn{3}{l|}{\textbf{Transcript Named Entities}} & \multicolumn{2}{l}{\textbf{Tags}}   \\ \hline
% Entity                        & \#    & Label            & Entity                          & \#          & Label          & Entity                   & \#          & Label          & Tag                           & \#  \\ \hline
% Matt Christiansen             & 90    & PERSON           & Matt Christiansen               & 207         & PERSON         & Trump                    & 3125        & PERSON         & tenet media                   & 350 \\
% Dave Rubin \& Isabel Brown    & 89    & PERSON           & Dave Rubin                      & 132         & PERSON         & Joe Biden                & 1696        & PERSON         & entertainment                 & 306 \\
% Lauren Southern               & 68    & PERSON           & Chris Gard                      & 114         & PERSON         & Donald Trump             & 1465        & PERSON         & news                          & 159 \\
% Tayler Hansen                 & 44    & PERSON           & Trump                           & 93          & PERSON         & Biden                    & 1350        & PERSON         & dave rubin                    & 123 \\
% Tim Pool                      & 38    & PERSON           & Biden                           & 87          & PERSON         & America                  & 1203        & GPE            & matt christiansen             & 120 \\
% Biden                         & 21    & PERSON           & Brown                           & 85          & PERSON         & American                 & 1139        & NORP           & tenet                         & 115 \\
% Benny Johnson                 & 19    & PERSON           & Lauren Southern                 & 50          & PERSON         & Dave                     & 923         & PERSON         & isabel brown                  & 114 \\
% The Culture War               & 16    & EVENT            & Tim Pool                        & 45          & PERSON         & Democrats                & 786         & NORP           & reactions                     & 76  \\
% Trump                         & 11    & PERSON           & Connect                         & 44          & PERSON         & Kamala Harris            & 768         & PERSON         & lauren southern               & 74  \\
% Canada                        & 9     & GPE              & Tayler Hansen                   & 42          & PERSON         & Congress                 & 706         & ORG            & tim pool                      & 50  \\
% Benny Johnson \&              & 8     & ORG              & Benny Johnson                   & 41          & PERSON         & Florida                  & 590         & GPE            & the culture war               & 44  \\
% Kamala                        & 7     & PERSON           & Matt Christiansen Hour          & 29          & PERSON         & Tim                      & 572         & PERSON         & matt christiansen hour        & 41  \\
% Dave Rubin                    & 7     & PERSON           & Texas                           & 29          & GPE            & Democrat                 & 534         & NORP           & tayler hansen                 & 40  \\
% The Arena                     & 7     & WORK\_OF\_ART    & America                         & 29          & GPE            & California               & 508         & GPE            & joe biden                     & 33  \\
% The MC Hour                   & 6     & WORK\_OF\_ART    & FBI                             & 29          & ORG            & the United States        & 503         & GPE            & benny johnson                 & 30  \\
% America                       & 6     & GPE              & Joe Biden                       & 23          & PERSON         & Israel                   & 499         & GPE            & people of the internet        & 30  \\
% FBI                           & 6     & ORG              & California                      & 23          & GPE            & FBI                      & 492         & ORG            & donald trump                  & 28  \\
% Supreme Court                 & 6     & ORG              & Lisa Elizabeth                  & 22          & PERSON         & New York                 & 475         & GPE            & podcasts                      & 27  \\
% Frank                         & 5     & PERSON           & Isabel Brown                    & 21          & PERSON         & Americans                & 474         & NORP           & in the arena                  & 26  \\
% Joe Biden                     & 5     & PERSON           & Chicago                         & 20          & GPE            & Twitter                  & 473         & PRODUCT        & the culture war with tim pool & 22 
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \centering
% \begin{tabular}{lll|lll|ll}
% \multicolumn{3}{l|}{\textbf{Video Title Named Entities}} & \multicolumn{3}{l|}{\textbf{Video Description Named Entities}} & \multicolumn{2}{l}{\textbf{Tags}}   \\ \hline
% Entity                        & \#    & Label            & Entity                          & \#          & Label          & Tag                           & \#  \\ \hline
% Matt Christiansen             & 90    & PERSON           & Matt Christiansen               & 207         & PERSON         & tenet media                   & 350 \\
% Dave Rubin \& Isabel Brown    & 89    & PERSON           & Dave Rubin                      & 132         & PERSON         & entertainment                 & 306 \\
% Lauren Southern               & 68    & PERSON           & Chris Gard                      & 114         & PERSON         & news                          & 159 \\
% Tayler Hansen                 & 44    & PERSON           & Trump                           & 93          & PERSON         & dave rubin                    & 123 \\
% Tim Pool                      & 38    & PERSON           & Biden                           & 87          & PERSON         & matt christiansen             & 120 \\
% Biden                         & 21    & PERSON           & Brown                           & 85          & PERSON         & tenet                         & 115 \\
% Benny Johnson                 & 19    & PERSON           & Lauren Southern                 & 50          & PERSON         & isabel brown                  & 114 \\
% The Culture War               & 16    & EVENT            & Tim Pool                        & 45          & PERSON         & reactions                     & 76  \\
% Trump                         & 11    & PERSON           & Connect                         & 44          & PERSON         & lauren southern               & 74  \\
% Canada                        & 9     & GPE              & Tayler Hansen                   & 42          & PERSON         & tim pool                      & 50  \\
% Benny Johnson \&              & 8     & ORG              & Benny Johnson                   & 41          & PERSON         & the culture war               & 44  \\
% Kamala                        & 7     & PERSON           & Matt Christiansen Hour          & 29          & PERSON         & matt christiansen hour        & 41  \\
% Dave Rubin                    & 7     & PERSON           & Texas                           & 29          & GPE            & tayler hansen                 & 40  \\
% The Arena                     & 7     & WORK\_OF\_ART    & America                         & 29          & GPE            & joe biden                     & 33  \\
% The MC Hour                   & 6     & WORK\_OF\_ART    & FBI                             & 29          & ORG            & benny johnson                 & 30  \\
% America                       & 6     & GPE              & Joe Biden                       & 23          & PERSON         & people of the internet        & 30  \\
% FBI                           & 6     & ORG              & California                      & 23          & GPE            & donald trump                  & 28  \\
% Supreme Court                 & 6     & ORG              & Lisa Elizabeth                  & 22          & PERSON         & podcasts                      & 27  \\
% Frank                         & 5     & PERSON           & Isabel Brown                    & 21          & PERSON         & in the arena                  & 26  \\
% Joe Biden                     & 5     & PERSON           & Chicago                         & 20          & GPE            & the culture war with tim pool & 22 
% \end{tabular}
% \end{table*}
